Exploring GPU-to-GPU Communication: Insights into Supercomputer Interconnects

Multi-GPU nodes are increasingly common in the rapidly evolving landscape of exascale supercomputers. On these systems, GPUs on the same node are connected through dedicated networks, with bandwidths up to a few terabits per second. However, gauging performance expectations and maximizing system efficiency is challenging due to different technologies, design options, and software layers. This paper comprehensively characterizes three supercomputers - Alps, Leonardo, and LUMI - each with a unique architecture and design. We focus on performance evaluation of intra-node and inter-node interconnects on up to 4096 GPUs, using a mix of intra-node and inter-node benchmarks. By analyzing its limitations and opportunities, we aim to offer practical guidance to researchers, system architects, and software developers dealing with multi-GPU supercomputing. Our results show that there is untapped bandwidth, and there are still many opportunities for optimization, ranging from network to software optimization.

==> tables/table1.tex <==
{\scriptsize
\begin{tabularx}{\linewidth}{p{3cm}|X|X|X}
                 & {\centering \textbf{Alps}}     & {\centering\textbf{Leonardo}}             & {\centering\textbf{LUMI}}             \\ \hline
CPU              & 72-core NVIDIA \textit{Grace}  & 32-core Intel \textit{Ice Lake} Xeon 8358 & 64-core AMD \textit{Trento} EPYC 7A53 \\ \hline
GPU              & 4x NVIDIA \textit{Hopper} H100 & 4x NVIDIA \textit{Ampere} A100            & 4x AMD MI250X (8 GCDs)                \\ \hline
NICs             & 4x HPE Cray 200 Gb/s Cassini-1 & 2x dual-port NVIDIA Connect-X6 (100 Gb/s per port) (i.e., 4x 100 Gb/s ports) & 4x HPE Cray 200 Gb/s Cassini-1 \\ \hline 
Intra-node Interconnect & 6x NVLink 3.0 links towards any other GPU (1.2 Tb/s between any pair) & 4x NVLink 3.0 links towards any other GPU (800 Gb/s between any pair)  & Between 1 and 4 400 Gb/s Infinity Fabric links towards other GCDs (see Fig.~\ref{fig:lumi})     \\ \hline 
Inter-node Interconnect & HPE Cray Slingshot 11. Dragonfly topology & NVIDIA Infiniband HDR. Dragonfly+ topology with 23 groups. Each group is a 2-level \textit{Fat-tree} &  HPE Cray Slingshot 11. Dragonfly topology with 24 groups     \\ \hline
Software Envirorment &    Cray MPICH \texttt{v8.1.28}, libfabric \texttt{v1.15.2}, NVIDIA driver \texttt{v535.129.03}.                          & Open MPI \texttt{v4.1.4.4}, CUDA \texttt{v12.1}, NCCL \textcolor{red}{X.X} &  Cray clang \texttt{v16.0.1}, Cray MPICH \texttt{v8.1.27}, libfabric \texttt{v1.15.2}, ROCM \texttt{v5.2.3}, \texttt{aws-ofi-rccl} plugin (\texttt{v1.4}).  \\ 
\end{tabularx}
}

==> tables/table2.tex <==

%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\begin{tabular}{ c c c c c c c c c c c c c c }
\cline{1-14} \\[0.5ex]
\textbf{Reference} & \textbf{Accelerator} & \multicolumn{2}{c}{\textbf{Communication Primitive}} & \multicolumn{5}{c}{\textbf{Communication Library}} & \multicolumn{4}{c}{\textbf{Characterization}} & \makecell{\\ \textbf{Scale}\\\textbf{(GPU per node)}} \\ \cline{3-13} \\[0.1ex]
 &  & \textbf{P2P} & \textbf{Collectives} & \textbf{MPI} & \textbf{GPU-aware} & \textbf{*CCL} & \textbf{Fabric} & \textbf{Hybrid} & \textbf{P} & \textbf{AR} & \textbf{HC} & \textbf{NN} &  \\ 
\\[0.1ex]
%OK to check 
\rowcolor{lightgray!20} DeSensi~\cite{Desensi2020} & $\times$ & SR & A2A & \checkmark & $\times$ & $\times$ &  $\times$ & $\times$ & \checkmark & \checkmark &  $\times$ & \checkmark & $1024$ \\ \hline

%OK to check all-to-all, one- and two-sided
% incast, one- and two-sided broadcasts)
Atchley~\cite{10.1145/3581784.3607089} & AMD MI250x (2 GCD)  & SR & A2A, AR, AG & \checkmark & \checkmark & $\times$ &  \checkmark & $\times$ &  \checkmark & \checkmark &  $\times$ & \checkmark & $9400$ (4 GPUs) \\ \hline

%OK
\rowcolor{lightgray!20} Siefertl~\cite{10.1145/3624062.3624203} & \makecell{AMD MI250x (2 GCD)\\NVIDIA A100\\NVIDIA GV100} & SR & A2A & $\times$ & \checkmark & $\times$ &  \checkmark & $\times$ &  \checkmark & $\times$ &  $\times$ & $\times$ & $1$ (4 GPUs)\\ \hline

%OK
Khorassani.~\cite{khorassani2023high} & AMD MI100 & SR & A2A,AR,AG,SG,BC & \checkmark & \checkmark & \checkmark &  $\times$ & $\times$ &  \checkmark & $\times$ &  $\times$ & $\times$ & $16$(4 GPUs) \\ \hline

\rowcolor{lightgray!20}
Li~\cite{Li2020} & \makecell{NVIDIA P100 DGX-1\\NVIDIA V100 DGX-1\\NVIDIA V100 DGX-2} & SR & A2A,RS,BC & $\times$ & \checkmark & \checkmark &  \checkmark & $\times$ &  \checkmark & $\times$ &  $\times$ & $\times$ & $8$\footnote{Single node, up to 16 GPUs on DGX--2, while up to 6 on Summit}\\ \hline

Person~\cite{pearson2023interconnect}  &  AMD MI250x (2 GCD) & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &  \checkmark & $\times$ & \checkmark & $\times$ &  $\times$ & $\times$ & $1$ (4 GPUs) \\ \hline
 
\rowcolor{customcolor!40!white} \textbf{(This work)}  & \makecell{AMD MI250x (2 GCD)\\NVIDIA A100\\NVIDIA H100} & SR & A2A,AR,IC & \checkmark & \checkmark & \checkmark &  \checkmark & \checkmark &  \checkmark & \checkmark &  \checkmark & \checkmark & $512$ (8 GPUs) \\ \hline 


 
\end{tabular}

%%% Legend
% S=send R=receive iS iR
% A2A = All2ALL, AR = AllReduce IC=incast 


% MN = Multi-node
% LS large-scale 
% S 
